ProactiveAudioBench: Evaluating Condition-Driven Responses in Audio Streams

As multimodal models advance from offline understanding to real-time interaction, audio assistants must continuously monitor user-specified targets and respond proactively when the requested conditions are met. Existing evaluations, however, do not systematically cover the diverse listening targets and notification requirements across sound, speech, and music. We introduce ProactiveAudioBench, comprising four task families and 22 subtasks across these three domains, including pronunciation correction, tool calling, musical section tracking, and matching against reference audio. These tasks combine diverse listening targets with rules specifying notifications at the first, every, or $N$th qualifying occurrence, while also testing whether models remain silent when conditions are unmet. The benchmark contains 1,999 listening requests with reference notification times and responses, curated through automated checks and two-stage human review. Our evaluation framework supports both simulated and native streaming and jointly assesses notification timing and response content. Experiments across 23 model-interface configurations show that high event coverage does not ensure reliable execution of listening requests, as models struggle to avoid both omissions and extra outputs. Further diagnostics reveal limitations in event counting and temporal grounding even without autonomous notification timing, suggesting that reliable listening requires improvements in both rule execution and the underlying audio capabilities.

==> vendor/forloop/README <==
Description
-----------

The forloop package provides the command \forloop for the user.


Installation
------------

To install this package, run forloop.ins through LaTeX.  This will generate 
a file called forloop.sty.  Put this file somewhere where LaTeX will find 
it---for instance localtexmf/tex/latex/forloop/  (note that you will need 
to create the folder forloop).

If you are using MikTeX, you then need to refresh the file name database 
by using MikTeX Options


License
-------

This package is released under the GNU Lesser General Public License.  See
https://www.gnu.org/licenses/licenses.html#LGPL for more details.

Contact
-------

Any bugs may be reported to the author by sending an email to the
address with the first part being "latex", a dash, then "inquiries",
then an at sign, the next part is nsetzer, and finally it ends in dot com.


